Tracking Knowledge Propagation Across Wikipedia Languages

In this paper, we present a dataset of inter-language knowledge propagation in Wikipedia. Covering the entire 309 language editions and 33M articles, the dataset aims to track the full propagation history of Wikipedia concepts, and allow follow up research on building predictive models of them. For this purpose, we align all the Wikipedia articles in a language-agnostic manner according to the concept they cover, which results in 13M propagation instances. To the best of our knowledge, this dataset is the first to explore the full inter-language propagation at a large scale. Together with the dataset, a holistic overview of the propagation and key insights about the underlying structural factors are provided to aid future research. For example, we find that although long cascades are unusual, the propagation tends to continue further once it reaches more than four language editions. We also find that the size of language editions is associated with the speed of propagation. We believe the dataset not only contributes to the prior literature on Wikipedia growth but also enables new use cases such as edit recommendation for addressing knowledge gaps, detection of disinformation, and cultural relationship analysis.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections/KP_modeling.tex <==
\section{Modeling Knowledge Propagation}
\label{sec:modeling}

\begin{figure*}
      \input{figure/tikz/ex1}\hfill
      \input{figure/tikz/ex2}\hfill
      \input{figure/tikz/ex3}\hfill
      \input{figure/tikz/ex4}\hfill
    \caption{For a given item, the \emph{English} (EN), \emph{German} (DE), \emph{French} (FR), and \emph{Portuguese} (PT) pages were created at times $t_1 < t_2 < t_3 < t_4$, respectively.  An arrow from $X$ to $Y$ indicates direct influence from page $X$ to page $Y$. In Scenario (a), pages were created independently. In Scenarios (b)-(d), the page creator used/translated content from other pages.}
    \label{fig:propagex}
\end{figure*} 

In this section, we take a step further and develop a model to predict items' propagation. More specifically, given a partial history of page creations up to time $t$, we ask two questions:

\begin{enumerate}
    \item Will the propagation continue in the short term?
    \item Given that the propagation will continue, which are the most likely next language editions?
\end{enumerate}

Answering these questions would be difficult if pages are created in an independent manner. Even if there are strong patterns, the problem is challenging as we only have the timestamped sequence of page creations and the influence among language editions is invisible in the data. 
%is challenging because, from our dataset, we only know the sequence of timestamps when each page was created. For instance, if we observe page $Y$ appearing after page $X$, we do not know whether the appearance of page $Y$ was influenced by $X$.%, but this knowledge could be helpful for our task.
%In order to better explain the issue introduced in the previous paragraph, consider the example presented in Figure \ref{fig:propagex}. 
Figure \ref{fig:propagex} depicts the challenge by showing  four different scenarios for the same sequence of page creations. %regarding the creation of four pages related to the same item.
Figure \ref{subfig:propa} represents the case where the four pages were independently created, while Figures \ref{subfig:propb}-\ref{subfig:propd} represent scenarios 
in which there may have been influence between page creations (\emph{e.g.}, via direct translation or a follow up creation with richer information).

%From our data, \emph{i.e.}, sequence of pages and their respective creation times, one may be tempted to assume a linear chain of events, as depicted in Figure \ref{subfig:propb}, to describe the relationship among pages. Proceeding in this way can be misleading because such an assumptions does not take into account other important factors, such as: geography, cultural aspects, and language similarity.

Our approach to the absence of explicit links of interaction %causal knowledge 
is to use the whole dataset and infer the cascades from the sequence of observed language edition labels and timestamps \cite{netrapalli:2012,lishen:2016}. 
%Unfortunately, achieving a reasonable inference is hard and, in some cases, a nearly-impossible task {\color{red}We have a citation, right?}
We avoid making any assumption about the possible influence among page creations and frame the above two questions as a machine learning problem. 
%In order to answer questions (1) and (2), we opted for an approach that avoids making any explicit assumption with regard to the influence that a set of pages may have in the appearance of a new one. More specifically, we decided to frame those questions as machine learning problems.

\subsection{Model Description}

\begin{figure}[h]
    \input{figure/tikz/scheme}
    \caption{Overview of our prediction problems.}
    \label{fig:window}
\end{figure}

%In this section, we present the models for predicting whether a cascade will continue and if so, to predict the most likely languages to appear.
Figure \ref{fig:window} shows an overview of our prediction problems. For a given item, pages $P_1,\dots,P_L$ appeared at times $t_1,\dots,t_L$, respectively. Then, we want a model that, given the information about the last $K$ pages, predicts if a new page would appear, and in which language if it appears. 
%what happens to the propagation within a timeout period $\delta$. More specifically, will a new page appear? If so, which one?

\begin{figure}
  \input{figure/tikz/models}
  \caption{(a) model to decide whether propagation will continue; (b) model to identify likely languages to appear.}
  \label{fig:models}
\end{figure} 

Given the temporal nature of our data, we develop a model based on LSTM (Long Short-Term Memory) networks \cite{lstm:1997}. 
In Figure \ref{fig:models}, we show how we use LSTMs to create an architecture for each prediction problem. Note that our goal here is to examine the feasibility of prediction rather than to find the best possible models/architectures. 
%Our goal here is not to search for the best possible models/architectures, but to propose reasonable solutions.
The inputs for both models are the same, i.e., the models are aware of the last $K$ pages and the time difference between the appearance of each page and its predecessor.
With these inputs, the model could learn 
%Our intuition for considering this input is to allow the models to understand 
not only the sequences, but the propagation speed as well. %(see examples of different propagation speeds in Figure \ref{fig:example-cascades}). We added a second LSTM layer to the second model, once predicting the next language is a harder problem, which is a multi-class classification task. 
As for the second task, another LSTM layer is added to the model since the task is a more difficult,  multi-class classification problem.  

The output of the first model is a probability: if it is greater than 0.5, the model predicts that a new page will appear within the timeout $\delta$.
The second model outputs a probability distribution over all languages. Then, the language with the maximum probability is chosen. %In this case, the model's prediction is the most probable language to appear next in the sequence. 
In this last step we exclude the languages that already appeared in the sequence, because each cascade can have only a single instance of a language. % just one article associated to a given Wikidata item. 

\subsection{Model Evaluation}

To evaluate the models' performance, we split our dataset into two parts, using older data for training and newer data for testing. 
The training set is collected from the items created between January 1st, 2008, and  January 1st, 2015. As mentioned above, the year 2008 is selected since most of the languages were present in Wikipedia from the year. 
%that starting year considering at that point 
There were already 10M articles in 251 languages (Figure \ref{fig:langsPerYear}\footnote{\url{https://en.wikipedia.org/wiki/History_of_Wikipedia}}). The test set includes the items created after January 1st, 2015. %Therefore, items/sequences used to train the model were not used to test the model. 
We train a binary model for the first task with nearly 200 thousand instances (randomly sampled), in batch size of 2000 instances and 20 epochs, and a validation split of 10\%. The parameters were empirically chosen regarding the 
%We empirically chose these parameters based on 
the available data and the performance. 
The same set of parameters are used for the second task, 
%In the task of predicting the next language, we used the same parameters, 
except the number of epochs. The number of epochs is increased to 200 considering the higher complexity of the task. 
%which we increased to 200. The number of epochs is chosen considering the accuracy during the training process. The investigation of the possibility of propagating is a task less complex than investigating the most likely languages to propagate. It requires fewer epochs to converge to an acceptable level. 

The choice of the timeout, $\delta$, for the first task involves a trade-off: a value too small skews the data with negative labels whereas the opposite would skew the data with positive labels. We set $\delta$ as one year, in order to make the prediction task intuitive and to avoid the skew (the ratio of positive and negative labels is around 3:7). 
%We considered the timeout, $\delta$, value as one year. We chose $\delta$ with the objective that our training data do not become highly unbalanced. By selecting a period of one year, the ratio of cascades propagating over not propagating is around 3/7. 
We test the model with more than 20 thousand instances. 

The input window size, $K$, also involves a trade-off: a window too small cannot provide meaningful signal to the model whereas the opposite can use only long propagation instances and significantly reduces the available data as a consequence. For both tasks, We set $K = 4$, which gave a reasonable balance. 

%For both models, we considered the $K = 4$, i.e.; we used information about the last four pages to predict what happens next. The selection of a K=4 took into consideration the number of cascades with at least K+1 languages available in the dataset. The number of cascades should be sufficient to train the model. Also, the used cascade should have enough information to feed the model. Therefore, the size selection needs to compromise between having bigger cascades and smaller samples available.

\begin{table}[h]
    \caption{Binary classification results}
    \label{tab:binres}
    \begin{tabular}{cccc}
    \hline
    \hline
    \textbf{Class} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} \\
    \hline
    Not propagate     & 0.99 & 0.96 & 0.98 \\
    Propagate     & 0.96 & 0.99 & 0.98 \\
    \hline
    \hline
    \end{tabular}
\end{table}

Table \ref{tab:binres} presents the results of our binary model, demonstrating the %where one can observe that distinguishing items whose propagation will continue or not is a 
feasibility of the task (with high accuracy).
%As shown in Figure \ref{fig:predictionacc}, 
However, predicting the next language is much more challenging. 
Our model made an accurate prediction for about 9\% of the test cases. While the result 
%We observe that our model was able to pinpoint the exact next language in around the 9\% of the test cases, which 
is much better than a random guess (\~0.3\%), it is obvious that the performance is worse than that of the first model. 
%not as good as the binary classification described before. 
Figure \ref{fig:predictionacc} shows an additional analysis of the performance where we relax the evaluation criteria and allow a window of error, \textit{i.e.}, to check if the predicted language is included in the window of next languages. The performance quickly improves with the increase of the error window $w$, and it reaches about 30\% when the window size is 5. 
%in approximately 30\% of the test cases. %In 65\% of the cases, our prediction did not appear in the remaining of the sequence.

Despite additional trials with increased complexity of the model ( more layers and units), we did not see significant improvements. 
%In order to investigate the limitation of the last result, we increased the complexity of the model, adding more layers and units. However, the improvements were not significant. 
While we believe that the results imply the existence of meaningful patterns, they also suggest that future investigation is necessary considering additional information and different representations of the data. 
%In future work, we intend to investigate how to improve this model by considering different information and/or different representation of the data.

\begin{figure}
    \centering
    \includegraphics[scale=1]{figure/acc-real-data.pdf}
    \caption{Next language prediction results.}
    \label{fig:predictionacc}
\end{figure}


==> sections/introduction.tex <==
\section{Introduction}
\sloppy
Increasing global connectivity and digital tools foster knowledge propagation in all aspects; frequency, reach, and directions. Wikipedia is one of the key platform for knowledge propagation, especially between its language editions. The unique features of Wikipedia, such as wide language coverage, extensiveness of topics, and large-scale collaborative participation, provide an opportunity to track the knowledge propagation taking in place of the platform. The structural factors within Wikipedia, for example, cultural/linguistic similarity \textcolor{red}{[]}, distribution of multi-lingual editors\textcolor{red}{[]}, topics of common international interests \textcolor{red}{[]} also suggest the possibility to model and predict knowledge propagation. 

In this paper, we develop a dataset to capture inter-language knowledge propagation in Wikipedia. 
%provide a comprehensive overview of knowledge propagation in Wikipedia, and examine predictive models of the propagation.
%Covering the whole language editions and entire Wikipedia page creations, 
The data set tracks knowledge propagation by aligning the entire page creations in a language agnostic manner. The sequence of page creations across the whole language editions is aggregated for every Wikipedia item. Figure~\ref{fig:example-cascades} shows some example propagation instances, a few showing a bursty expansion and a few showing a steady growth. 

%\textcolor{red}{
%Note the continuous propagation on relevant timeless themes (i.e.: Artificial Intelligence, Naan) or popular figures (i.e.: Tom Jobim and LeBron James), and a bursting behaviour on trending themes (i.e.: Fake News and Michel Teló) }
%\todo[]{Reference to Figure 1 here?}


\textcolor{red}{Can we save some of this paragraph for future publication?} To the best of our knowledge, this dataset is the first to view the growth of Wikipedia from the perspective of inter-language propagation. 


Through this dataset, we aim to promote future research on data-driven modeling and prediction of knowledge propagation. 


Many recent works~\cite{wulczyn2016growing,mcdonough2015revision,kaffee2018mind} aim at promoting such interactions in order to expedite the growth of Wikipedia. Our work also pays attention to the interactions and attempt to provide a holistic view. 

We believe that the dataset presented in this work can be used, as main object of study or complementary material, by researchers from many areas. The applications may range from conducting in-depth exploratory analyses (e.g., multilingual behavior in Wikipedia and topic/temporal similarities between languages) to building systems capable of predicting the the next language that a Wikipedia page will appear or recommending pages to be written in a given language.

% \textcolor{red}{While the notion of knowledge propagation could be seen similar to information diffusion, language editions or editors in Wikipedia are not connected in a network structure and the interactions between them are not explicit unlike, for example, in online social networks where sending and reception of information is often visible. }
% Wikipedia does offer a direct translation tool, which captures the interaction between language editions; however, we find that the usage of the tool account for a small fraction of page creations. 
% \textcolor{red}{Many works have been made around the diffusion in networks, looking into the different types and process of diffusion regarding the network structure \cite{goel2012structure}, and the possibility of making predictions \cite{cheng2014can}.} %Despite the absence of a network structure, we believe similar approaches can be made to model knowledge propagation considering possible structural factors within Wikipedia, for example, cultural/linguistic similarity, distribution of multi-lingual editors, topics of common international interests. 
\begin{figure}[ht]
\centering
    %\includegraphics[width=0.96\linewidth]{figure/example-cascades.pdf}
    % WARNING: If we try to increase this figure, hell breaks loose
    \includegraphics[scale=0.59]{figure/example-cascades.pdf}
    \caption{Example propagation across Wikipedia language editions.}
    \label{fig:example-cascades}
\end{figure}

% Clearly, articles of different languages in Wikipedia are not necessarily (and not usually) translations of each other, and often include different content. 
% Each Wikipedia language edition is built by its own community, using different sources, taking different perspectives, and covering at different depths even for equivalent concepts. Having strong local and independent communities supports the creation of diverse content and prevents imposing point of views coming from a particular language edition. However, this also creates knowledge gaps between projects \cite{wulczyn2016growing}, frequently missing content from one language edition in others. 
% Previous research has observed small overlaps among language editions \cite{hecht2009measuring}, and also that even large projects, such as English Wikipedia, are not a super-set of all the knowledge in all Wikis \cite{hecht2013mining}. 
% Yet, the differences among the language editions do not imply that they grow independently.

...

The structural factors mentioned above create interactions and make them influence each other. 

Many recent works~\cite{wulczyn2016growing,mcdonough2015revision,kaffee2018mind} aim at promoting such interactions in order to expedite the growth of Wikipedia. Our work also pays attention to the interactions and attempt to provide a holistic view. % \textcolor{red}{I reordered the two recovered sentences and merged a bit with others. Does it seem okay?}
...

Through this dataset, we aim to promote future research on data-driven modeling and prediction of knowledge propagation. 

For this objective, various exploratory analyses are presented. 
%regarding the reach, speed, ordering among language editions, and topics. The results reveal both challenges and opportunities for modeling the propagation. 
%consistent to the finding in information diffusion networks, we observe a highly skewed distribution; 
For example, we observe that only a small fraction of items propagate to many language editions, consistent to the finding made in social networks \cite{goel2012structure}; however, propagation is more common in Wikipedia.
%In addition, simple associations between propagation and individual language editions or topics are hardly found, for example, Wikipedia items of greater propagation are covered by diverse different editions rather than being covered by large, popular language editions. 
The propagation tends to gain speed, suggesting the possibility to predict whether an item would further propagate or not. We also find association between the size of language editions and the speed of propagation. 
%We also observe more frequent propagation among language editions that show higher cultural and linguistic similarity, which corroborates the findings made in prior works on multi-lingual editors \cite{samoilenko2016linguistic}, coverage of popular figures \cite{eom2015interactions}.

%Aggregating all propagation instances of every Wikipedia item, we explore Structural patterns in relation to the language editions involved in the propagation and the topics of the items.

The remainder of this paper is organized as follows: first, we briefly discuss the related work; next we explain how we collected and prepared the dataset; then, we present some basic statistics and characteristics of the data and use cases where such a dataset can be useful. Finally, we present our conclusions and discuss future work.

% \begin{itemize}
% \item Our view of Wikipedia as a unique platform where we can observe knowledge propagation across language editions. 
%     \begin{itemize}
%         \item 309 different languages (e.g., English, Portuguese, and Catalan) hosted
%         \item The importance of understanding the growth and interaction of language editions in wikipedia.
%         \item possible mechanisms of interaction?
%         \item Impact of understanding the mechanisms?
%     \end{itemize}
% \item Our approach to understand and model knowledge propagation, taking a network perspective. 
%     \begin{itemize}
%         \item Language editions do not have an explicit network structure, but there are underlying factors 
%         \item cultural and linguistic similarity and distances
%         \item multi-lingual editors
%     \end{itemize}
% \item Result 1. Overview of knowledge propagation in Wikipedia
% \item Result 2. Development and Evaluation of a propagation model

%\end{itemize}
